Hallucination-Aware Generative Pretrained Transformer for Cooperative Aerial Mobility Control

This paper proposes SafeGPT, a two-tiered framework that integrates generative pretrained transformers (GPTs) with reinforcement learning (RL) for efficient and reliable unmanned aerial vehicle (UAV) last-mile deliveries. In the proposed design, a Global GPT module assigns high-level tasks such as sector allocation, while an On-Device GPT manages real-time local route planning. An RL-based safety filter monitors each GPT decision and overrides unsafe actions that could lead to battery depletion or duplicate visits, effectively mitigating hallucinations. Furthermore, a dual replay buffer mechanism helps both the GPT modules and the RL agent refine their strategies over time. Simulation results demonstrate that SafeGPT achieves higher delivery success rates compared to a GPT-only baseline, while substantially reducing battery consumption and travel distance. These findings validate the efficacy of combining GPT-based semantic reasoning with formal safety guarantees, contributing a viable solution for robust and energy-efficient UAV logistics.

==> Table/Table_training.tex <==
\begin{tabularx}{1\linewidth}{l c c c}
    \toprule[1pt]
%     \multicolumn{4}{c}{\textbf{\circled{1} : Performance when action dimension is $|\mathcal{A}| = 2^{16}$}} \\
% \toprule[1pt]

Algorithm & QoS  & Capacity & Residual Energy \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 

\textbf{QMARL}
& $\mathbf{0.874}$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.874,0) -- (0.974,0);
\draw[black,line width=1pt] (0.874,-2pt) -- (0.874,2pt);
\draw[black,line width=1pt] (0.974,-2pt) -- (0.974,2pt);}
& $\mathbf{0.871}$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.871,0) -- (0.971,0);
\draw[black,line width=1pt] (0.871,-2pt) -- (0.871,2pt);
\draw[black,line width=1pt] (0.971,-2pt) -- (0.971,2pt);}
& $\mathbf{0.872}$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.872,0) -- (0.972,0);
\draw[black,line width=1pt] (0.872,-2pt) -- (0.872,2pt);
\draw[black,line width=1pt] (0.972,-2pt) -- (0.972,2pt);} \\

MARL
& $0.468$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.468,0) -- (0.568,0);
\draw[black,line width=1pt] (0.468,-2pt) -- (0.468,2pt);
\draw[black,line width=1pt] (0.568,-2pt) -- (0.568,2pt);}
& $0.394$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.394,0) -- (0.494,0);
\draw[black,line width=1pt] (0.394,-2pt) -- (0.394,2pt);
\draw[black,line width=1pt] (0.494,-2pt) -- (0.494,2pt);}
& $0.471$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.471,0) -- (0.571,0);
\draw[black,line width=1pt] (0.471,-2pt) -- (0.471,2pt);
\draw[black,line width=1pt] (0.571,-2pt) -- (0.571,2pt);} \\

IQL
& $0.143$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.143,0) -- (0.243,0);
\draw[black,line width=1pt] (0.143,-2pt) -- (0.143,2pt);
\draw[black,line width=1pt] (0.243,-2pt) -- (0.243,2pt);}
& $0.228$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.228,0) -- (0.328,0);
\draw[black,line width=1pt] (0.228,-2pt) -- (0.228,2pt);
\draw[black,line width=1pt] (0.328,-2pt) -- (0.328,2pt);}
& $0.419$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.419,0) -- (0.519,0);
\draw[black,line width=1pt] (0.419,-2pt) -- (0.419,2pt);
\draw[black,line width=1pt] (0.519,-2pt) -- (0.519,2pt);} \\

DQN
& $0.183$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.183,0) -- (0.283,0);
\draw[black,line width=1pt] (0.183,-2pt) -- (0.183,2pt);
\draw[black,line width=1pt] (0.283,-2pt) -- (0.283,2pt);}
& $0.289$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.289,0) -- (0.389,0);
\draw[black,line width=1pt] (0.289,-2pt) -- (0.289,2pt);
\draw[black,line width=1pt] (0.389,-2pt) -- (0.389,2pt);}
& $0.439$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.439,0) -- (0.539,0);
\draw[black,line width=1pt] (0.439,-2pt) -- (0.439,2pt);
\draw[black,line width=1pt] (0.539,-2pt) -- (0.539,2pt);} \\


Random
& $0.145$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.145,0) -- (0.245,0);
\draw[black,line width=1pt] (0.145,-2pt) -- (0.145,2pt);
\draw[black,line width=1pt] (0.245,-2pt) -- (0.245,2pt);}
& $0.238$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.238,0) -- (0.338,0);
\draw[black,line width=1pt] (0.238,-2pt) -- (0.238,2pt);
\draw[black,line width=1pt] (0.338,-2pt) -- (0.338,2pt);}
& $0.441$\; \tikz{
\draw[gray,line width=.3pt] (0,0) -- (1.1,0);
\draw[white, line width=0.01pt] (0,-2pt) -- (0,2pt);
\draw[black,line width=1pt] (0.441,0) -- (0.541,0);
\draw[black,line width=1pt] (0.441,-2pt) -- (0.441,2pt);
\draw[black,line width=1pt] (0.541,-2pt) -- (0.541,2pt);} \\

\bottomrule[1pt]
\end{tabularx}
